PITA: Physics-Informed Trajectory Autoencoder

Validating robotic systems in safety-critical appli-cations requires testing in many scenarios including rare edgecases that are unlikely to occur, requiring to complement real-world testing with testing in simulation. Generative models canbe used to augment real-world datasets with generated data toproduce edge case scenarios by sampling in a learned latentspace. Autoencoders can learn said latent representation for aspecific domain by learning to reconstruct the input data froma lower-dimensional intermediate representation. However, theresulting trajectories are not necessarily physically plausible, butinstead typically contain noise that is not present in the inputtrajectory. To resolve this issue, we propose the novel Physics-Informed Trajectory Autoencoder (PITA) architecture, whichincorporates a physical dynamics model into the loss functionof the autoencoder. This results in smooth trajectories that notonly reconstruct the input trajectory but also adhere to thephysical model. We evaluate PITA on a real-world dataset ofvehicle trajectories and compare its performance to a normalautoencoder and a state-of-the-art action-space autoencoder.

==> figs/table_paramters.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Models} & $\lambda_1$ & $\lambda_2$ & $\step$ \\
\hline
$\pita_{\text{recon}}$ & ? & ? & ? \\
$\pita_{\text{smooth}}$ & ? & ? & ? \\
\hline
\end{tabular}
\caption{Comparison of model parameters for the three autoencoder models.}
\label{tab:hyperparameters}
\end{table*}
